SAFREE: Training-Free and Adaptive Guard for Safe Text-to-Image And Video Generation

Recent advances in diffusion models have significantly enhanced their ability to generate high-quality images and videos, but they have also increased the risk of producing unsafe content. Existing unlearning/editing-based methods for safe generation remove harmful concepts from models but face several challenges: (1) They cannot instantly remove harmful concepts without training. (2) Their safe generation capabilities depend on collected training data. (3) They alter model weights, risking degradation in quality for content unrelated to toxic concepts. To address these, we propose SAFREE, a novel, training-free approach for safe T2I and T2V, that does not alter the model's weights. Specifically, we detect a subspace corresponding to a set of toxic concepts in the text embedding space and steer prompt embeddings away from this subspace, thereby filtering out harmful content while preserving intended semantics. To balance the trade-off between filtering toxicity and preserving safe concepts, SAFREE incorporates a novel self-validating filtering mechanism that dynamically adjusts the denoising steps when applying the filtered embeddings. Additionally, we incorporate adaptive re-attention mechanisms within the diffusion latent space to selectively diminish the influence of features related to toxic concepts at the pixel level. In the end, SAFREE ensures coherent safety checking, preserving the fidelity, quality, and safety of the output. SAFREE achieves SOTA performance in suppressing unsafe content in T2I generation compared to training-free baselines and effectively filters targeted concepts while maintaining high-quality images. It also shows competitive results against training-based methods. We extend SAFREE to various T2I backbones and T2V tasks, showcasing its flexibility and generalization. SAFREE provides a robust and adaptable safeguard for ensuring safe visual generation.

==> materials/fig_intro.tex <==
\begin{wrapfigure}{rt}{0.4\textwidth}  % Right side, takes up 0.5 of text width
\vspace{-0.1in}
  \begin{minipage}{\linewidth}   % First figure (half width)
    \centering
    \includegraphics[width=\linewidth]{assets/distance_toxicity.pdf}  % Replace with your figure path
    \vspace{-0.25in}
    \caption{Correlation between toxicity prediction and distance to the target concept subspace.}
    \label{fig:embedding_stats}
  \vspace{0.1in}
  \end{minipage}
  \begin{minipage}{\linewidth}   % Second figure (half width)
    \centering
    \includegraphics[width=\linewidth]{assets/intro.pdf}  % Replace with your figure path
    \vspace{-0.25in}
    \caption{Gaussian distributions of the distance between the nudity subspace and Ring-a-bell or COCO 30k prompts.}\label{fig:embedding_stats_gaussian}    
  \end{minipage}
    \vspace{-0.9in}
\end{wrapfigure}

==> materials/figure_unsafe.tex <==
\begin{figure*}[t]
    \centering
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{cccc}
        \includegraphics[width=0.22\textwidth]{assets/SD-v1-4-vangogh.pdf}&
    \includegraphics[width=0.22\textwidth]{assets/CA-vangogh.pdf}&
    \includegraphics[width=0.22\textwidth]{assets/RECE-vangogh.pdf}&
    \includegraphics[width=0.22\textwidth]{assets/ours-vangogh.pdf}
\\
         \textbf{(a) SD}&
         \textbf{(b) CA}&
         \textbf{(c) RECE}&
         \textbf{(d) \ours{} (Ours)}
         
% \vspace{0.05in}\\
    \end{tabular}}
    
    \caption{\textbf{Qualitative Analysis of Safe Generation} Images will be updated later
    }
    \label{fig:artist}

\end{figure*}

==> materials/table_ablation.tex <==
% \begin{table*}
% \caption{Ablation Study.}\label{tab:t2i_ablation}
% \small
% \centering
% \setlength{\tabcolsep}{1.mm}
% \resizebox{0.6\textwidth}{!}{
% \begin{tabular}{ l | c c c | c c | c c} % \multicolumn{4}{c}{}
% \toprule
% &&&&\multicolumn{2}{c}{\textbf{Adversarial Prompts}}&\multicolumn{2}{c}{\textbf{COCO-30K}}\\ 
% \textbf{Method}&\textbf{Token}&\textbf{Balancing}&\textbf{Latent}& \textbf{P4D} $\downarrow$ &\textbf{MMA-Diffusion} $\downarrow$ & \textbf{FID} $\downarrow$ & \textbf{CLIP} $\uparrow$\\
% \hline
% SD-v1-4&-&-&-&0.987& 0.957 &-&  31.3\\
% \hline
% \multirow{5}{*}{\begin{tabular}~\ours{}\\(Ours)\end{tabular}}
% % &Dense&-&-&0.436&0.268&45.6& 31.4&0.38&0.813\\
% &Null&-&-&0.430&\textbf{0.512}&37.6&30.9\\
% &Projection&-&-&0.417&0.597&36.5& \underline{31.1}\\
% &Projection&$\checkmark$&-&	&0.598	&\textbf{29.1}&	\textbf{31.4}\\
% &Projection&-&$\checkmark$&0.410&0.588&42.2&30.7\\
% &Projection&$\checkmark$&$\checkmark$&\textbf{0.384}&\underline{0.585}&\underline{36.4}&\underline{31.1}\\
% \bottomrule
% \end{tabular}
% }
% \end{table*}








% \begin{table*}
% \caption{Ablation Study.}\label{tab:t2i_ablation}
% \small
% \centering
% \setlength{\tabcolsep}{1.mm}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{ l | c c c | c c | c c | c c }
% \toprule
% \multicolumn{4}{c}{}&\multicolumn{2}{c}{Adversarial Prompts}&\multicolumn{2}{c}{COCO-30K}&\multicolumn{2}{c}{Artists}\\ 
% Method&Token&Balancing&Latent&P4D $\downarrow$ &MMA-Diffusion $\downarrow$ &FID $\downarrow$ & CLIP $\uparrow$ & {ER. Acc.} $\downarrow$ & {Un. Acc.} $\uparrow$\\
% \midrule
% SD-v1-4&-&-&-&0.987& 0.957 &-&  31.3&0.875&0.888\\
% \midrule
% \multirow{5}{*}{\begin{tabular}~\ours{}\\(Ours)\end{tabular}}
% % &Dense&-&-&0.436&0.268&45.6& 31.4&0.38&0.813\\
% &Null&-&-&0.430&\textbf{0.512}&37.6&30.9&0.275&0.738\\
% &Projection&-&-&0.417&0.597&36.5& \underline{31.1}& 0.400 & 0.775\\
% &Projection&$\checkmark$&-&	&0.598	&\textbf{29.1}&	\textbf{31.4}\\
% &Projection&-&$\checkmark$&0.410&0.588&42.2&30.7&\\
% &Projection&$\checkmark$&$\checkmark$&\textbf{0.384}&\underline{0.585}&\underline{36.4}&\underline{31.1}\\
% \bottomrule
% \end{tabular}
% }
% \end{table*}

==> materials/table_baselines.tex <==
\begin{table*}
\caption{\textbf{Comparison of our approach with recent safe vision generation methods.} Most of the work is primarily designed to prevent the generalization of toxic images by modifying the weights of the pre-trained diffusion model. These methods lack versatility (deploying different diffusion models, image editing, and video generation tasks, etc.), and are vulnerable to multimodal attacks and/or multiple controls.}\label{tab:baselines}
\setlength{\tabcolsep}{2mm}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lcccccccccccc}
\toprule
\textbf{Methods} & \textbf{Publications} & \textbf{Generation Task} & \textbf{Image Filter} & \textbf{Video Filter} & \textbf{Text Filter} & \textbf{Training-Free} & \textbf{Model Agnostic}\\ \midrule
DALL$\cdot$E 3~\citep{2023dalle3} & - & Text-to-Image & \textcolor{Green}{\cmark} & \xmark & \textcolor{Green}{\cmark} & \textcolor{Green}{\cmark} & \xmark\\
SLD~\citep{schramowski2023safe} & CVPR 23' & Text-to-Image & \xmark & \xmark & \xmark & \textcolor{Green}{\cmark} & \xmark\\
ESD~\citep{gandikota2023erasing} & ICCV 23' & Text-to-Image & \xmark & \xmark & \xmark & \xmark & \xmark\\
UCE~\citep{liu2024rethinking} & & Text-to-Image & \xmark & \xmark & \xmark & \xmark & \xmark\\
TBD\\
TBD\\
TBD\\
TBD\\
% Ethic-Lens~\citep{cai2024ethical} & arXiv 24.04 & Text-to-Image & \textcolor{Green}{\cmark} & \xmark & \textcolor{Green}{\cmark} & \xmark & \textcolor{Green}{\cmark}\\
\midrule
\textbf{\ours{}} (Ours) & - & Text-to-Image/Video &\multicolumn{3}{c}{[\textcolor{Green}{\cmark}~Multimodal Compositional Safety Filter]} & \textcolor{Green}{\cmark} & \textcolor{Green}{\cmark}\\
\bottomrule
\vspace{-.1in}
\end{tabular}}
\end{table*}

==> materials/tables_old.tex <==
\begin{table*}
\caption{Attack Success Rate, SP: Subspace Proximity, NB: Negative Prompt Balance, $^\dagger$: from RECE}\label{tab:t2i_main}
\small
\centering
\setlength{\tabcolsep}{1.mm}
\resizebox{\textwidth}{!}{
\begin{tabu}{lc|ccccc|cc}
\toprule
& &\multirow{3}{*}{I2P $\downarrow$}&\multirow{3}{*}{P4D $\downarrow$}&\multirow{3}{*}{Ring-A-Bell $\downarrow$}&\multirow{3}{*}{MMA-Diffusion $\downarrow$}&\multirow{3}{*}{UnlearnDiffAtk $\downarrow$}&\multicolumn{2}{c}{COCO-30k}\\ 
\cmidrule(lr){8-9}
Method&Publication&
&&&&&FID $\downarrow$ &CLIP $\uparrow$\\
\midrule
SD-v1.4 &-&
0.570&
0.987&0.831$^\dagger$&&&14.5&31.3\\
% SD-v2.0 &-&&0.960&&&&&\\
SDXL &-&
\todo{}&
0.709&&&
&&\\
\midrule
\rowfont{\color{mygray}}
{ESD~\citep{gandikota2023erasing}} &{ICCV 23'} &
\todo{}&\todo{}
&0.528&0.873&0.761
&15.9&30.7\\
\rowfont{\color{mygray}}
{MACE~\citep{lu2024mace}}&{CVPR 24'} &
\todo{}&\todo{}\\
\rowfont{\color{mygray}}
{SDID~\citep{li2024self}}&{CVPR 24'} &0.270\\
\rowfont{\color{mygray}}
{Latent Guard~\citep{liu2024latent}}&{ECCV 24'} &{no}&code\\
\midrule
NGPT~\citep{Woolf2023} & - &
\todo{}&\todo{}&&&
&&\\
SLD-Medium~\citep{schramowski2023safe} &CVPR 23' &
\todo{}&0.592&&&
&16.9&31.0$^\dagger$
\\
SLD-Max~\citep{schramowski2023safe} &CVPR 23'&
\todo{}&0.775$^\dagger$&0.662$^\dagger$&&0.824$^\dagger$
&18.8&\\
UCE~\citep{gandikota2024unified}&WACV 24' &
0.253&
0.803$^\dagger$&0.331$^\dagger$&\todo{0.367}&0.796$^\dagger$
&15.7&31.3$^\dagger$\\
% T2IShield~\citep{wang2024t2ishield}&ECCV 24' &\\
% \rowfont{\color{mygray}}SafeGen~\citep{li2024safegen}&CCS 24'&data&gen&is needed&-&-&-&-\\
% NGPT-Lazy~\citep{ban2024understanding} &arXiv 24.06 &
% &
% 0.007&&&
% &&\\
SA~\citep{heng2023selective}&NeurIPS 23'&
&0.789$^\dagger$&0.225$^\dagger$&&0.775$^\dagger$&&30.6$^\dagger$\\
CA~\citep{kumari2023ablating}&ICCV 23'&&\textbf{0.606}$^\dagger$&0.254$^\dagger$&&0.655$^\dagger$&&31.2$^\dagger$\\
RECE~\citep{gong2024reliable}&ECCV 24' &
\textbf{0.092}&0.649$^\dagger$&\textbf{0.134}$^\dagger$&&0.655$^\dagger$&&30.9$^\dagger$\\
% RECE~\citep{gong2024reliable}&ECCV 24' &0.190&0.649$^\dagger$&\textbf{0.134}$^\dagger$&&0.655$^\dagger$&&30.9$^\dagger$\\
\rowfont{\color{mygray}}
{ConceptPrune~\citep{chavhan2024conceptprune}}&{arXiv 24.05}&&&
0.148&0.044&\textbf{0.648}
&16.9&29.9\\
\midrule
\rowfont{\color{mygray}}
SD-v1.4 Coco Subsample&-
&&&&&&&30.9\\
\midrule
% \ours~(Ours): SP-$\alpha=0.005$ (denoising: 0-49)&-
% &\todo{0.197}&\todo{}&\todo{0.076}&&&\todo{}&\todo{30.4}\\
% \ours~(Ours): SP-$\alpha=0.0$ (denoising: 0-49)&-
% &\todo{\textbf{0.070}}&\todo{0.193}&\todo{0.038}&&&\todo{}&\todo{25.7}\\
% \ours~(Ours): SP-$\alpha=0.0$ + NB&-&\todo{}&\todo{}&\todo{}&&&\todo{}&\todo{}\\
\ours~(Ours): SP-$\alpha=0.0$ (denoising: 0-4)&-&\todo{}&\todo{}&\todo{0.139}&&0.190&\todo{}&\todo{30.6}\\
\rowfont{\color{azure(colorwheel)}}{\ours~(Ours): SP-$\alpha=0.0$ (denoising: 0-9)}&-&\todo{}&\todo{}&{\textbf{0.038}}&&0.092&\todo{}&{30.0}\\
{\ours~(Ours): SP-$\alpha=0.0$ (denoising: 0-14)}&-&\todo{}&\todo{}&{\textbf{0.013}}&&0.056&\todo{}&\todo{{29.7}}\\
\ours~(Ours): SP-$\alpha=0.0$-null (denoising: 0-4)&-&&&0.051&&&&30.5\\
% {\ours~(Ours): SP-$\alpha=0.0$-null (denoising: 0-9)}&-&&&&&&&\\
\rowfont{\color{azure(colorwheel)}}\ours~(Ours): SP-$\alpha=0.0$-ONP (denoising: 0-4)&-&&&0.101&&&&{\textbf{31.1}}\\
% {\ours~(Ours): SP-$\alpha=0.0$-ONP (denoising: 0-9)}&-&&&0.076&&&&30.4\\
\ours~(Ours): SP-$\alpha=0.0$-M2O (denoising: 0-4)&-&&&0.089&&&&30.6\\
% {\ours~(Ours): SP-$\alpha=0.0$-M2O (denoising: 0-9)}&-&&&&&&&30.6\\
\ours~(Ours): SP-$\alpha=0.01$-M2O (denoising: 0-4)&-&&&0.051&&&&30.7\\
% {\ours~(Ours): SP-$\alpha=0.01$-M2O (denoising: 0-9)}&-&&&0.076&&&&30.7\\
\bottomrule
\end{tabu}
}
\end{table*}



\begin{table*}
\caption{Attack Effectiveness.}\label{tab:3d_main}
\small
\centering
\setlength{\tabcolsep}{1.mm}
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccc}
\toprule
&
\multicolumn{7}{c}{I2P}&
NSFW\\ 
\cmidrule(lr){2-8} \cmidrule(lr){9-9}
Method&
Hate&
Harassment&
Violence&
Self-harm&
Sexual&
Shocking&
Illegal Activity\\ 
\midrule
VideoCrafter2\\
+ Toxigen\\
+ NSFW text classifier\footnote{https://huggingface.co/michellejieli/NSFW_text_classifier}\\
+ SD safety checker\footnote{https://huggingface.co/CompVis/stable-diffusion-safety-checker}\\
% + SD-NEGP~\cite{}\\
% + SLD-Medium~\cite{} \\
% + SLD-Strong~\cite{} \\
% + SLD-Max~\cite{} \\
% + ESD~\cite{} \\
\midrule
T2V-turbo\\
+ Toxigen\\
+ NSFW text classifier\\
+ SD safety checker\\
% SD-NEGP~\cite{}\\
% SLD-Medium~\cite{} \\
% SLD-Strong~\cite{} \\
% SLD-Max~\cite{} \\
% ESD~\cite{} \\
\midrule
\ours~(Ours)\\

\bottomrule
\end{tabular}}
\end{table*}

% \begin{table*}
% \caption{Attack Effectiveness. IVA Bench: Inappropriate Video Action Bench}\label{tab:3d_main}
% \small
% \centering
% \setlength{\tabcolsep}{1.mm}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{lccccccccc}
% \toprule
% Method&
% Shocking&
% Illegial&
% Violance&
% Sexual&
% Racism&
% GPT-4v&
% CLIP-Text &
% Aesthetic\\ 
% \midrule
% % SD 1.5~\cite{}\\
% % SD 2.0~\cite{}\\
% % SD-NEGP~\cite{}\\
% % SLD-Weak~\cite{} \\
% % SLD-Strong~\cite{} \\
% % SLD-Max~\cite{} \\
% % ESD~\cite{} \\
% VideoCrafter2\\
% T2V-Turbo\\
% \midrule
% \ours~(Ours)\\

% \bottomrule
% \end{tabular}}
% \end{table*}




==> olds/3_method_old.tex <==
\begin{table*}
\caption{Attack Success Rate, SP: Subspace Proximity, NB: Negative Prompt Balance, $^\dagger$: from RECE}\label{tab:t2i_main}
\small
\centering
\setlength{\tabcolsep}{1.mm}
\resizebox{\textwidth}{!}{
\begin{tabu}{lc|ccccc|ccc}
\toprule
& &\multirow{3}{*}{I2P $\downarrow$}&\multirow{3}{*}{P4D $\downarrow$}&\multirow{3}{*}{Ring-A-Bell $\downarrow$}&\multirow{3}{*}{MMA-Diffusion $\downarrow$}&\multirow{3}{*}{UnlearnDiffAtk $\downarrow$}&\multicolumn{3}{c}{COCO-30k}\\ 
\cmidrule(lr){8-10}
Method&Publication&
&&&&&FID $\downarrow$ &CLIP $\uparrow$&TIFA $\uparrow$\\
\midrule
SD-v1.4 &-&
0.570&
0.987&0.831$^\dagger$&0.957&0.697&14.5&31.3\\
SDXL &-&
run&
0.709&run&run&run
&-&-\\
\midrule
\rowfont{\color{mygray}}
{ESD~\citep{gandikota2023erasing}} &{ICCV 23'} &
\todo{}&\todo{}
&0.528&0.873&0.761
&15.9&30.7\\
\rowfont{\color{mygray}}
{MACE~\citep{lu2024mace}}&{CVPR 24'} &
\todo{}&\todo{}\\
\rowfont{\color{mygray}}
{SDID~\citep{li2024self}}&{CVPR 24'} &0.270\\
\rowfont{\color{mygray}}
{Latent Guard~\citep{liu2024latent}}&{ECCV 24'} &{no}&code\\
\midrule
NGPT~\citep{Woolf2023} & - &
&&&&
&&30.7\\
SLD-Medium~\citep{schramowski2023safe} &CVPR 23' &
\todo{}&0.592&&&
&16.9&31.0$^\dagger$
\\
SLD-Max~\citep{schramowski2023safe} &CVPR 23'&
\todo{}&0.775$^\dagger$&0.662$^\dagger$&&0.824$^\dagger$
&18.8&\\
UCE~\citep{gandikota2024unified}&WACV 24' &
0.253&
0.803$^\dagger$&0.331$^\dagger$&\todo{0.367}&0.796$^\dagger$
&15.7&31.3$^\dagger$\\
% T2IShield~\citep{wang2024t2ishield}&ECCV 24' &\\
% \rowfont{\color{mygray}}SafeGen~\citep{li2024safegen}&CCS 24'&data&gen&is needed&-&-&-&-\\
SA~\citep{heng2023selective}&NeurIPS 23'&
0.621$^*$ &0.789$^\dagger$&0.225$^\dagger$&&0.775$^\dagger$&&30.6$^\dagger$\\
CA~\citep{kumari2023ablating}&ICCV 23'& 0.226$^*$&\textbf{0.606}$^\dagger$&0.254$^\dagger$&0.855$^*$&0.655$^\dagger$&&31.2$^\dagger$\\
RECE~\citep{gong2024reliable}&ECCV 24' &
\textbf{0.092}&0.649$^\dagger$&\textbf{0.134}$^\dagger$&&0.655$^\dagger$&&30.9$^\dagger$\\
\rowfont{\color{mygray}}
{ConceptPrune~\citep{chavhan2024conceptprune}}&{arXiv 24.05}&&&
0.148&0.044&\textbf{0.648}
&16.9&29.9\\
\midrule
\rowfont{\color{mygray}}
SD-v1.4 Coco Subsample&-
&&&&&&&30.9\\
\midrule
% \ours~(Ours): SP-$\alpha=0.0$ (denoising: 0-4)&-&\todo{}&\todo{}&\todo{0.139}&&0.190&\todo{}&\todo{30.6}\\
% \rowfont{\color{azure(colorwheel)}}{\ours~(Ours): SP-$\alpha=0.0$ (denoising: 0-9)}&-&\todo{}&\todo{}&{\textbf{0.038}}&&0.092&\todo{}&{30.0}\\
% {\ours~(Ours): SP-$\alpha=0.0$ (denoising: 0-14)}&-&\todo{}&\todo{}&{\textbf{0.013}}&&0.056&\todo{}&\todo{{29.7}}\\
% \ours~(Ours): SP-$\alpha=0.0$-null (denoising: 0-4)&-&&&0.051&&&&30.5\\
\ours~(Ours): ONP&-&\textbf{0.028}&run&0.101&run&{0.384}&&{\textbf{31.1}}\\
\ours~(Ours): M2O, $\alpha=0.01$&-&0.035&&\textbf{0.051}&run&\todo{0.374}&&30.7\\
\bottomrule
\end{tabu}
}
\end{table*}


% \ours~(Ours): ONP&-&0.028&run&0.101&run&{0.268}&&{\textbf{31.1}}\\
% \ours~(Ours): SP-$\alpha=0.0$-M2O (denoising: 0-4)&-&&&0.089&&&&30.6\\
% \ours~(Ours): M2O, $\alpha=0.01$&-&0.035&&\textbf{0.051}&run&\todo{0.261}––––&&30.7\\


% I2P - M2O /nas-ssd2/jhyoon/safe_vidgen/P4D/results/run_0903_SDv1-4_std_artists_VanGogh_big_artist_tfg_alpha_0p01_M2O_0to4
% I2P - ONP /nas-ssd2/jhyoon/safe_vidgen/P4D/results/run_0902_SDv1-4_std_artists_VanGogh_big_artist_tfg_alpha_0p002_ONP_0to4
